TRIDENT: A load-balancing Clos-network Packet Switch with Queues between Input and Central Stages and In-Order Forwarding

We propose a three-stage load balancing packet switch and its configuration scheme. The input- and central-stage switches are bufferless crossbars, and the output-stage switches are buffered crossbars. We call this switch ThRee-stage Clos-network swItch with queues at the middle stage and DEtermiNisTic scheduling (TRIDENT), and the switch is cell based. The proposed configuration scheme uses predetermined and periodic interconnection patterns in the input and central modules to load-balance and route traffic, therefore; it has low configuration complexity. The operation of the switch includes a mechanism applied at input and output modules to forward cells in sequence. TRIDENT achieves 100% throughput under uniform and nonuniform admissible traffic with independent and identical distributions (i.i.d.). The switch achieves this high performance using a low-complexity architecture while performing in-sequence forwarding and no central-stage expansion or memory speedup. Our discussion includes throughput analysis, where we describe the operations the configuration mechanism performs on the traffic traversing the switch, and proof of in-sequence forwarding. We present a simulation analysis as a practical demonstration of the switch performance under uniform and nonuniform i.i.d. traffic.

==> Reference.tex <==
@inproceedings{chrysos2006scheduling,
  title={Scheduling in Non-Blocking Buffered Three-Stage Switching Fabrics.},
  author={Chrysos, Nikolaos and Katevenis, Manolis},
  booktitle={INFOCOM},
  volume={6},
  pages={1--13},
  year={2006}
}
@inproceedings{kleban2007modified,
  title={The modified {MSM} {C}los switching fabric with efficient packet dispatching scheme},
  author={Kleban, Janusz and Sobieraj, Maciej and Weclewski, Slawomir},
  booktitle={High Performance Switching and Routing, 2007. HPSR'07. Workshop on},
  pages={1--6},
  year={2007},
  organization={IEEE}
}

@inproceedings{kleban2013static,
  title={Static dispatching with internal backpressure scheme for {SMM} {C}los-network switches},
  author={Kleban, Janusz and Suszynska, Urszula},
  booktitle={Computers and Communications (ISCC), 2013 IEEE Symposium on},
  pages={000654--000658},
  year={2013},
  organization={IEEE}
}

@article{sule2018split,
	title={A Split-Central-Buffered Load-Balancing Clos-Network Switch With In-Order Forwarding},
	author={Sule, Oladele Theophilus and Rojas-Cessa, Roberto and Dong, Ziqian and Lin, Chuan-Bi},
	journal={IEEE/ACM Transactions on Networking},
	year={2018},
	publisher={IEEE}
}

@article{theo2018split,
	title={A Split-Central-Buffered Load-Balancing Clos-Network Switch with In-Order Forwarding},
	author={Sule, Oladele Theophilus and Rojas-Cessa, Roberto and Dong, Ziqian and Lin, Chuan-Bi},
	journal={arXiv preprint arXiv:1812.11650},
	year={2018}
}

@inproceedings{pun2002static,
	title={Static round-robin dispatching schemes for Clos-network switches},
	author={Pun, Konghong and Hamdi, Mounir},
	booktitle={High Performance Switching and Routing, 2002. Merging Optical and IP Technologies. Workshop on},
	pages={329--333},
	year={2002},
	organization={IEEE}
}

@article{li2001enhanced,
	title={Enhanced Birkhoff-von Neumann decomposition algorithm for input queued switches},
	author={Li, J and Ansari, N},
	journal={IEE Proceedings-Communications},
	volume={148},
	number={6},
	pages={339--342},
	year={2001},
	publisher={IET}
}

@inproceedings{dixit2013impact,
  title={On the impact of packet spraying in data center networks},
  author={Dixit, Advait and Prakash, Pawan and Hu, Y Charlie and Kompella, Ramana Rao},
  booktitle={INFOCOM, 2013 Proceedings IEEE},
  pages={2130--2138},
  year={2013},
  organization={IEEE}
}

@INPROCEEDINGS{lb-virtual-topologies, 
author={S. M. Irteza and H. M. Bashir and T. Anwar and I. A. Qazi and F. R. Dogar}, 
booktitle={IEEE INFOCOM 2017 - IEEE Conference on Computer Communications}, 
title={Load balancing over symmetric virtual topologies}, 
year={2017}, 
volume={}, 
number={}, 
pages={1-9}, 
keywords={routing protocols;software defined networking;telecommunication network topology;telecommunication traffic;trees (mathematics);SAPS;SDN-based scheme;Symmetric Adaptive Packet Spraying;asymmetric topologies;bisection bandwidth;load balancing algorithm;multirooted trees;packet spraying;symmetric topologies;symmetric virtual topologies;Bandwidth;Conferences;Load management;Network topology;Spraying;Switches;Topology}, 
doi={10.1109/INFOCOM.2017.8057002}, 
ISSN={}, 
month={May},}

@inproceedings{mhamdi2003cbf,
	title={CBF: A high-performance scheduling algorithm for buffered crossbar switches},
	author={Mhamdi, Lotfi and Hamdi, Mounir},
	booktitle={High Performance Switching and Routing, 2003, HPSR. Workshop on},
	pages={67--72},
	year={2003},
	organization={IEEE}
}

@ARTICLE{multipath-switching-slice12, 
author={L. Shi and B. Liu and C. Sun and Z. Yin and L. N. Bhuyan and H. J. Chao}, 
journal={IEEE Transactions on Computers}, 
title={Load-Balancing Multipath Switching System with Flow Slice}, 
year={2012}, 
volume={61}, 
number={3}, 
pages={350-365}, 
keywords={file organisation;probability;resource allocation;MPS;core routers;flow slice;flow-based hashing algorithms;load-balancing multipath switching system;petabit switching capacity;probability;Complexity theory;Context;Delay;Hardware;Switches;Switching systems;Upper bound;Load balancing;switching theory.;traffic measurement}, 
doi={10.1109/TC.2010.279}, 
ISSN={0018-9340}, 
month={March},}

@article{kermani1979virtual,
  title={Virtual cut-through: A new computer communication switching technique},
  author={Kermani, Parviz and Kleinrock, Leonard},
  journal={Computer Networks (1976)},
  volume={3},
  number={4},
  pages={267--286},
  year={1979},
  publisher={Elsevier}
}

@article{birkhoff1946tres,
  title={Tres observaciones sobre el algebra lineal},
  author={Birkhoff, Garrett},
  journal={Univ. Nac. Tucum{\'a}n Rev. Ser. A},
  volume={5},
  pages={147--151},
  year={1946}
}

@misc{lozowick1994method,
  title={Method and apparatus for cut-through data packet transfer in a bridge device},
  author={Lozowick, Philip P and Ben-Michael, Siman-Tov},
  year={1994},
  month=apr # "~26",
  publisher={Google Patents},
  note={US Patent 5,307,345}
}


@article{crrd,
  author =       {E. Oki and Z. Jing and R. Rojas-Cessa and H.J. Chao},
  title =        {Concurrent round-robin-based dispatching schemes for {C}los-network switches},
  journal =    {IEEE/ACM Trans. on Networking.},
  volume=        {10},
  number=        {6},
  year =         {2002},
  pages=         {830-844}
}


@article{rojas2004ufpim,
  title={Captured-frame eligibility and round-robin matching for input-queued packet switches},
  author={Rojas-Cessa, Roberto and Lin, Chuan-Bi},
  journal={IEEE communications letters},
  volume={8},
  number={9},
  pages={585--587},
  year={2004},
  publisher={IEEE}
}

@article{rojas2007captured,
  title={Captured-frame matching schemes for scalable input-queued packet switches},
  author={Rojas-Cessa, Roberto and Lin, Chuan-Bi},
  journal={Computer Communications},
  volume={30},
  number={10},
  pages={2149--2161},
  year={2007},
  publisher={Elsevier}
}

@INPROCEEDINGS{cixb, 
author={R. Rojas-Cessa and E. Oki and Zhigang Jing and H. J. Chao}, 
booktitle={High Performance Switching and Routing, 2001 IEEE Workshop on}, 
title={{CIXB}-1: combined input-one-cell-crosspoint buffered switch}, 
year={2001}, 
pages={324-329}, 
keywords={buffer storage;computational complexity;delays;packet switching;queueing theory;telecommunication traffic;timing;CIXB-1;buffer size;buffered crossbars;combined input-one-cell-crosspoint buffered switch;delay performance;fixed size packets;memory technology;packet switching;pin count;round-robin arbitration;scalability;simulation;switch architecture;switch module;switching throughput;time complexity;timing relaxation;uniform traffic;virtual output queues;Bandwidth;Buffer storage;Chaos;Delay;Fabrics;Rail to rail outputs;Scalability;Switches;Throughput;Traffic control}, 
doi={10.1109/HPSR.2001.923655}, 
}

@inproceedings{cixob,
  title={{CIXOB}-k: Combined input-crosspoint-output buffered packet switch},
  author={Rojas-Cessa, Roberto and Oki, Eiji and Chao, H Jonathan},
  booktitle={Global Telecommunications Conference, 2001. GLOBECOM'01. IEEE},
  volume={4},
  pages={2654--2660},
  year={2001},
  organization={IEEE}
}

@inproceedings{li2005space,
	title={Space-memory-memory architecture for Clos-network packet switches},
	author={Li, Xin and Zhou, Zhen and Hamdi, Mounir},
	booktitle={Communications, 2005. ICC 2005. 2005 IEEE International Conference on},
	volume={2},
	pages={1031--1035},
	year={2005},
	organization={IEEE}
}
@article{ clos1953study,
  title={A Study of Non-Blocking Switching Networks},
  author={Clos, Charles},
  journal={Bell System Technical Journal},
  volume={32},
  number={2},
  pages={406--424},
  year={1953},
  publisher={Wiley Online Library}
}

@article{chang2002load,
  title={Load balanced {B}irkhoff--von {N}eumann switches, part I: one-stage buffering},
  author={Chang, Cheng-Shang and Lee, Duan-Shin and Jou, Yi-Shean},
  journal={Computer Communications},
  volume={25},
  number={6},
  pages={611--622},
  year={2002},
  publisher={Elsevier}
}

@article{changload,
  title={Load balanced {B}irkhoff-von {N}eumann switches, part II: Multi-stage buffering},
  author={Chang, Cheng-Shang and Lee, Duan-Shin and Lien, Ching-Ming},
  publisher={Elsevier}
}

@incollection{ma2007analysis,
  title={Analysis on memory-space-memory {C}los packet switching network},
  author={Ma, Xiangjie and Hu, Yuxiang and Mao, Junpeng and Lan, Julong and Guan, Lian and Zhang, Baisheng},
  booktitle={Advanced Parallel Processing Technologies},
  pages={209--221},
  year={2007},
  publisher={Springer}
}


@inproceedings{rojas2006scalable,
  title={Scalable two-stage {C}los-network switch and module-first matching},
  author={Rojas-Cessa, Roberto and Lin, Chuan-Bi},
  booktitle={2006 Workshop on High Performance Switching and Routing},
  pages={6--pp},
  year={2006},
  organization={IEEE}
}

@article{oki2002concurrent,
  title={Concurrent round-robin-based dispatching schemes for {C}los-network switches},
  author={Oki, Eiji and Jing, Zhigang and Rojas-Cessa, Roberto and Chao, H Jonathan},
  journal={Networking, IEEE/ACM Transactions on},
  volume={10},
  number={6},
  pages={830--844},
  year={2002},
  publisher={IEEE}
}

@inproceedings{oki2009analysis,
  title={Analysis of space-space-space {C}los-network packet switch},
  author={Oki, Eiji and Kitsuwan, Nattapong and Rojas-Cessa, Roberto},
  booktitle={Computer Communications and Networks, 2009. ICCCN 2009. Proceedings of 18th International Conference on},
  pages={1--6},
  year={2009},
  organization={IEEE}
}

@inproceedings{rojas2004maximum,
  title={Maximum weight matching dispatching scheme in buffered {C}los-network packet switches},
  author={Rojas-Cessa, Roberto and Oki, Eiji and Chao, H Jonathan},
  booktitle={Communications, 2004 IEEE International Conference on},
  volume={2},
  pages={1075--1079},
  year={2004},
  organization={IEEE}
}


@inproceedings{dong2012mcs,
  title={{MCS}: buffered {C}los-network switch with in-sequence packet forwarding},
  author={Dong, Ziqian and Rojas-Cessa, Roberto},
  booktitle={Sarnoff Symposium (SARNOFF), 2012 35th IEEE},
  pages={1--6},
  year={2012},
  organization={IEEE}
}

@inproceedings{lin2013minimizing,
  title={Minimizing scheduling complexity with a {C}los-network space-space-memory ({SSM}) packet switch},
  author={Lin, Chuan-Bi and Rojas-Cessa, Roberto},
  booktitle={High Performance Switching and Routing (HPSR), 2013 IEEE 14th International Conference on},
  pages={15--20},
  year={2013},
  organization={IEEE}
}

@inproceedings{dong2011non,
  title={Non-blocking memory-memory-memory {C}los-network packet switch},
  author={Dong, Ziqian and Rojas-Cessa, Roberto},
  booktitle={34th IEEE Sarnoff Symposium},
  pages={1--5},
  year={2011},
  organization={IEEE}
}


@article{hu2010feedback,
  title={Feedback-based scheduling for load-balanced two-stage switches},
  author={Hu, Bing and Yeung, Kwan L},
  journal={IEEE/ACM Transactions on Networking (TON)},
  volume={18},
  number={4},
  pages={1077--1090},
  year={2010},
  publisher={IEEE Press}
}


@article{zhang2014space,
  title={Space-memory-memory {C}los-network switches with in-sequence service},
  author={Zhang, Maosen and Qiu, Zhiliang and Gao, Ya},
  journal={Communications, IET},
  volume={8},
  number={16},
  pages={2825--2833},
  year={2014},
  publisher={IET}
}

@inproceedings{dong2011memory,
  title={Memory-memory-memory {C}los-network packet switches with in-sequence service},
  author={Dong, Ziqian and Rojas-Cessa, Roberto and Oki, Eiji},
  booktitle={High Performance Switching and Routing (HPSR), 2011 IEEE 12th International Conference on},
  pages={121--125},
  year={2011},
  organization={IEEE}
}

@article{chao2003matching,
  title={Matching algorithms for three-stage bufferless {C}los network switches},
  author={Chao, H Jonathan and Jing, Zhigang and Liew, Soung Y},
  journal={Communications Magazine, IEEE},
  volume={41},
  number={10},
  pages={46--54},
  year={2003},
  publisher={IEEE}
}


@article{xia2016practical,
  title={A practical large-capacity three-stage buffered {C}los-network switch architecture},
  author={Xia, Yu and Hamdi, Mounir and Chao, H Jonathan},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={27},
  number={2},
  pages={317--328},
  year={2016},
  publisher={IEEE}
}

@inproceedings{hassen2017high,
  title={High-Capacity {C}los-Network Switch for Data Center Networks},
  author={Hassen, Fadoua and Mhamdi, Lotfi},
  booktitle={IEEE International Conference on Communications 2017},
  year={2017},
  organization={IEEE}
}

@article{lee1997path,
  title={Path switching-a quasi-static routing scheme for large-scale {ATM} packet switches},
  author={Lee, Tony T. and Lam, Cheuk H.},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={15},
  number={5},
  pages={914--924},
  year={1997},
  publisher={IEEE}
}
@inproceedings{chao2005trueway,
  title={Trueway: a highly scalable multi-plane multi-stage buffered packet switch},
  author={Chao, H Jonathan and Park, Jinsoo and Artan, Sertac and Jiang, Shi and Zhang, Guansong},
  booktitle={High Performance Switching and Routing, 2005. HPSR. 2005 Workshop on},
  pages={246--253},
  year={2005},
  organization={IEEE}
}

@article{atlanta,
  title={Low-cost scalable switching solutions for broadband networking: the {ATLANTA} architecture and chipset},
  author={Chiussi, Fabio M and Kneuer, Joseph G and Kumar, Vijay P},
  journal={IEEE Communications Magazine},
  volume={35},
  number={12},
  pages={44--53},
  year={1997},
  publisher={IEEE}
}

@inproceedings{keslassy2002maintaining,
  title={Maintaining packet order in two-stage switches},
  author={Keslassy, Isaac and McKeown, Nick},
  booktitle={INFOCOM 2002. Twenty-First Annual Joint Conference of the IEEE Computer and Communications Societies. Proceedings. IEEE},
  volume={2},
  pages={1032--1041},
  year={2002},
  organization={IEEE}
}

@book{rojas2016interconnections,
  title={Interconnections for Computer Communications and Packet Networks},
  author={Rojas-Cessa, Roberto},
  year={2016},
  publisher={CRC Press}
}

@article{lee1996new,
	title={A new decomposition algorithm for rearrangeable Clos interconnection networks},
	author={Lee, Hyun Yeop and Hwang, Frank K and Carpinelli, John D},
	journal={IEEE Transactions on Communications},
	volume={44},
	number={11},
	pages={1572--1578},
	year={1996},
	publisher={IEEE}
}

@inproceedings{hu2008joint,
	title={On joint sequence design for feedback-based two-stage switch architecture},
	author={Hu, Bing and Yeung, Kwan L},
	booktitle={High Performance Switching and Routing, 2008. HSPR 2008. International Conference on},
	pages={110--115},
	year={2008},
	organization={IEEE}
}

@inproceedings{mekkittikul1998practical,
	title={A practical scheduling algorithm to achieve 100\% throughput in input-queued switches},
	author={Mekkittikul, Adisak and McKeown, Nick},
	booktitle={INFOCOM'98. Seventeenth Annual Joint Conference of the IEEE Computer and Communications Societies. Proceedings. IEEE},
	volume={2},
	pages={792--799},
	year={1998},
	organization={IEEE}
}

@book{bertsekas1992data,
	title={Data networks},
	author={Bertsekas, Dimitri P and Gallager, Robert G and Humblet, Pierre},
	volume={2},
	year={1992},
	publisher={Prentice-Hall International New Jersey}
}

@article{little1961proof,
	title={A proof for the queuing formula: L= $\lambda$ W},
	author={Little, John DC},
	journal={Operations research},
	volume={9},
	number={3},
	pages={383--387},
	year={1961},
	publisher={INFORMS}
}

@article{chan1997pollaczek,
	title={Pollaczek-Khinchin formula for the M/G/1 queue in discrete time with vacations},
	author={Chan, WC and Lu, T-C and Chen, R-J},
	journal={IEE Proceedings-Computers and Digital Techniques},
	volume={144},
	number={4},
	pages={222--226},
	year={1997},
	publisher={IET}
}

@misc{bronshteinhandbook,
	title={Handbook of Mathematics. 2007},
	author={Bronshtein, IN and Semendyayev, KA and Musiol, G and Muehlig, H},
	publisher={Springer, Berlin}
}

@article{anderson1993high,
	title={High-speed switch scheduling for local-area networks},
	author={Anderson, Thomas E and Owicki, Susan S and Saxe, James B and Thacker, Charles P},
	journal={ACM Transactions on Computer Systems (TOCS)},
	volume={11},
	number={4},
	pages={319--352},
	year={1993},
	publisher={ACM}
}

@article{mckeown1993scheduling,
	title={Scheduling cells in an input-queued switch},
	author={McKeown, Nick and Varaiya, Pravin and Walrand, Jean},
	journal={Electronics Letters},
	volume={29},
	number={25},
	pages={2174--2175},
	year={1993},
	publisher={IET}
}

@article{karol1987input,
	title={Input versus output queueing on a space-division packet switch},
	author={Karol, Mark and Hluchyj, Michael and Morgan, Samuel},
	journal={IEEE Transactions on communications},
	volume={35},
	number={12},
	pages={1347--1356},
	year={1987},
	publisher={IEEE}
}

@article{karol1987input,
	title={Input versus output queueing on a space-division packet switch},
	author={Karol, Mark and Hluchyj, Michael and Morgan, Samuel},
	journal={IEEE Transactions on communications},
	volume={35},
	number={12},
	pages={1347--1356},
	year={1987},
	publisher={IEEE}
}

@phdthesis{mckeown1995scheduling,
	title={Scheduling algorithms for input-queued cell switches},
	author={McKeown, Nicholas William},
	year={1995},
	school={University of California, Berkeley}
}

@article{mekkittikul1997scheduling,
	title={Scheduling VOQ switches under non-uniform traffic},
	author={Mekkittikul, Adisak and McKeown, Nick},
	journal={CSL Technical Report, CSL-TR 97-747},
	year={1997},
	publisher={Citeseer}
}

@inproceedings{dai2000throughput,
	title={The throughput of data switches with and without speedup},
	author={Dai, JG and Prabhakar, Balaji},
	booktitle={INFOCOM 2000. Nineteenth Annual Joint Conference of the IEEE Computer and Communications Societies. Proceedings. IEEE},
	volume={2},
	pages={556--564},
	year={2000},
	organization={IEEE}

}

@inproceedings{mekkittikul1996starvation,
	title={A starvation-free algorithm for achieving 100\% throughput in an input-queued switch},
	author={Mekkittikul, Adisak and McKeown, Nick},
	booktitle={Proc. ICCCN},
	volume={96},
	pages={226--231},
	year={1996},
	organization={Citeseer}
}

@article{jenq1983performance,
	title={Performance analysis of a packet switch based on single-buffered banyan network},
	author={Jenq, Yih-Chyun},
	journal={IEEE Journal on Selected Areas in Communications},
	volume={1},
	number={6},
	pages={1014--1021},
	year={1983},
	publisher={IEEE}
}

@article{dong2012throughput,
	title={Throughput analysis of shared-memory crosspoint buffered packet switches},
	author={Dong, Ziqian and Rojas-Cessa, Roberto},
	journal={IET communications},
	volume={6},
	number={9},
	pages={1045--1053},
	year={2012},
	publisher={IET}
}

@inproceedings{rojas2006combined,
	title={Combined Input-Crosspoint Buffered Packet Switch with Flexible Access to Crosspoints Buffers},
	author={Rojas-Cessa, Roberto and Dong, Ziqian},
	booktitle={Devices, Circuits and Systems, Proceedings of the 6th International Caribbean Conference on},
	pages={255--260},
	year={2006},
	organization={IEEE}
}

@inproceedings{shah2002delay,
	title={Delay bounds for approximate maximum weight matching algorithms for input queued switches},
	author={Shah, Devavrat and Kopikare, Milind},
	booktitle={INFOCOM 2002. Twenty-First Annual Joint Conference of the IEEE Computer and Communications Societies. Proceedings. IEEE},
	volume={2},
	pages={1024--1031},
	year={2002},
	organization={IEEE}
}

@article{bastin2007lyapunov,
	title={Lyapunov stability analysis of networks of scalar conservation laws},
	author={Bastin, Georges and Haut, Bertrand and Coron, Jean-Michel and d Andrea-Novel, Brigitte},
	journal={Networks and Heterogeneous media},
	volume={2},
	number={4},
	pages={749},
	year={2007},
	publisher={AMERICAN INSTITUTE OF MATHEMATICAL SCIENCES}
}

@inproceedings{marsan2001packet,
	title={Packet scheduling in input-queued cell-based switches},
	author={Marsan, F Ajmone and Bianco, Andrea and Giaccone, Paolo and Leonardi, Emilio and Neri, E},
	booktitle={INFOCOM 2001. Twentieth Annual Joint Conference of the IEEE Computer and Communications Societies. Proceedings. IEEE},
	volume={2},
	pages={1085--1094},
	year={2001},
	organization={IEEE}
}

@article{dong2011buffered,
	title={Buffered clos-network packet switch with per-output flow queues},
	author={Dong, Ziqian and Rojas-Cessa, Roberto and Oki, Eiji},
	journal={Electronics letters},
	volume={47},
	number={1},
	pages={32--34},
	year={2011},
	publisher={IET}
}

@inproceedings{cai2011avoiding,
	title={Avoiding speedup from bandwidth overhead in a practical output-queued packet switch},
	author={Cai, Lin and Rojas-Cessa, Roberto and Kijkanjanarat, Taweesak},
	booktitle={Communications (ICC), 2011 IEEE International Conference on},
	pages={1--5},
	year={2011},
	organization={IEEE}
}

@article{chuang1999matching,
	title={Matching output queueing with a combined input/output-queued switch},
	author={Chuang, Shang-Tse and Goel, Ashish and McKeown, Nick and Prabhakar, Balaji},
	journal={IEEE Journal on Selected Areas in Communications},
	volume={17},
	number={6},
	pages={1030--1039},
	year={1999},
	publisher={IEEE}
}

@inproceedings{charny1998algorithms,
	title={Algorithms for providing bandwidth and delay guarantees in input-buffered crossbars with speedup},
	author={Charny, Anna and Krishna, P and Patel, Naimish and Simcoe, Robert},
	booktitle={Quality of Service, 1998.(IWQoS 98) 1998 Sixth International Workshop on},
	pages={235--244},
	year={1998},
	organization={IEEE}
}

@article{krishna1999speedup,
	title={On the speedup required for work-conserving crossbar switches},
	author={Krishna, Pattabhiraman and Patel, Naimish S and Charny, Anna and Simcoe, Robert J},
	journal={IEEE Journal on Selected Areas in Communications},
	volume={17},
	number={6},
	pages={1057--1066},
	year={1999},
	publisher={IEEE}
}

@article{prabhakar1999speedup,
	title={On the speedup required for combined input-and output-queued switching},
	author={Prabhakar, Balaji and McKeown, Nick},
	journal={Automatica},
	volume={35},
	number={12},
	pages={1909--1920},
	year={1999},
	publisher={Elsevier}
}

@inproceedings{stephens1998implementing,
	title={Implementing Distributed Packet Fair Queueing in a scalable switch architecture},
	author={Stephens, Donpaul C and Zhang, Hui},
	booktitle={INFOCOM'98. Seventeenth Annual Joint Conference of the IEEE Computer and Communications Societies. Proceedings. IEEE},
	volume={1},
	pages={282--290},
	year={1998},
	organization={IEEE}
}

@article{hluchyj1988queueing,
	title={Queueing in high-performance packet switching},
	author={Hluchyj, Michael G and Karol, Mark J},
	journal={IEEE Journal on selected Areas in Communications},
	volume={6},
	number={9},
	pages={1587--1597},
	year={1988},
	publisher={IEEE}
}

@inproceedings{iliadis1990performance,
	title={Performance of packet switches with input and output queueing},
	author={Iliadis, Ilias and Denzel, WOLFGANG E},
	booktitle={Communications, 1990. ICC'90, Including Supercomm Technical Sessions. SUPERCOMM/ICC'90. Conference Record., IEEE International Conference on},
	pages={747--753},
	year={1990},
	organization={IEEE}
}

@article{pattavina1993analysis,
	title={Analysis of input and output queueing for nonblocking ATM switches},
	author={Pattavina, Achille and Bruzzi, Giacomo},
	journal={IEEE/ACM Transactions on Networking (TON)},
	volume={1},
	number={3},
	pages={314--328},
	year={1993},
	publisher={IEEE Press}
}

@inproceedings{mckeown1997matching,
	title={Matching output queueing with combined input and output queueing},
	author={McKeown, Nick and Prabhakar, Balaji and Zhu, Mingyan},
	booktitle={PROCEEDINGS OF THE ANNUAL ALLERTON CONFERENCE ON COMMUNICATION CONTROL AND COMPUTING},
	volume={35},
	pages={595--603},
	year={1997},
	organization={Citeseer}
}

@article{del1993performance,
	title={Performance evaluation of input and output queueing techniques in ATM switching systems},
	author={Del Re, Enrico and Fantacci, Romano},
	journal={IEEE Transactions on communications},
	volume={41},
	number={10},
	pages={1565--1575},
	year={1993},
	publisher={IEEE}
}

@article{chen1993scoq,
	title={SCOQ: A fast packet switch with shared concentration and output queueing},
	author={Chen, David X and Mark, Jon W},
	journal={IEEE/ACM Transactions on Networking (TON)},
	volume={1},
	number={1},
	pages={142--151},
	year={1993},
	publisher={IEEE Press}
}

@article{rojas2011load,
	title={Load-balanced combined input-crosspoint buffered packet switches},
	author={Rojas-Cessa, Roberto and Dong, Ziqian},
	journal={IEEE Transactions on Communications},
	volume={59},
	number={5},
	pages={1421--1433},
	year={2011},
	publisher={IEEE}
}

@inproceedings{chang1999service,
	title={On service guarantees for input-buffered crossbar switches: a capacity decomposition approach by Birkhoff and von Neumann},
	author={Chang, Cheng-Shang and Chen, Wen-Jyh and Huang, Hsiang-Yi},
	booktitle={Quality of Service, 1999. IWQoS'99. 1999 Seventh International Workshop on},
	pages={79--86},
	year={1999},
	organization={IEEE}
}

@article{von1953certain,
	title={A certain zero-sum two-person game equivalent to the optimal assignment problem},
	author={Von Neumann, John},
	journal={Contributions to the Theory of Games},
	volume={2},
	pages={5--12},
	year={1953}
}

@inproceedings{chang2000birkhoff,
	title={Birkhoff-von Neumann input buffered crossbar switches},
	author={Chang, Cheng-Shang and Chen, Wen-Jyh and Huang, Hsiang-Yi},
	booktitle={IEEE INFOCOM. Nineteenth Annual Joint Conference of the IEEE Computer and Communications Societies. Proceedings. IEEE},
	volume={3},
	pages={1614--1623},
	year={2000},
	organization={IEEE}
}

@inproceedings{anderson1992high,
	title={High speed switch scheduling for local area networks},
	author={Anderson, Thomas E and Owicki, Susan S and Saxe, James B and Thacker, Charles P},
	booktitle={ACM SIGPLAN Notices},
	volume={27},
	number={9},
	pages={98--110},
	year={1992},
	organization={ACM}
}

@article{mckeown1999islip,
	title={The iSLIP scheduling algorithm for input-queued switches},
	author={McKeown, Nick},
	journal={IEEE/ACM transactions on networking},
	volume={7},
	number={2},
	pages={188--201},
	year={1999},
	publisher={IEEE}
}

@inproceedings{kanizo2009crosspoint,
	title={The crosspoint-queued switch},
	author={Kanizo, Yossi and Hay, David and Keslassy, Isaac},
	booktitle={INFOCOM 2009, IEEE},
	pages={729--737},
	year={2009},
	organization={IEEE}
}

@article{lin2005throughput,
	title={The throughput of a buffered crossbar switch},
	author={Lin, Mingjie and McKeown, Nick},
	journal={IEEE communications Letters},
	volume={9},
	number={5},
	pages={465--467},
	year={2005},
	publisher={IEEE}
}

@article{hu2016iterative,
	title={On Iterative Scheduling for Input-Queued Switches With a Speedup of $2-1/N$},
	author={Hu, Bing and Yeung, Kwan L and Zhou, Qian and He, Chunzhi},
	journal={IEEE/ACM Transactions on Networking},
	volume={24},
	number={6},
	pages={3565--3577},
	year={2016},
	publisher={IEEE}
}

@inproceedings{yan2014hybrid,
	title={Hybrid scheduling algorithm for packet switch architecture},
	author={Yan, Fangfang and Lee, Tony T and Ye, Tong and Hu, Weisheng},
	booktitle={Information Science, Electronics and Electrical Engineering (ISEEE), 2014 International Conference on},
	volume={1},
	pages={346--350},
	year={2014},
	organization={IEEE}
}

@article{rojas2006maximum,
	title={On the maximum throughput of a combined input-crosspoint queued packet switch},
	author={Rojas-Cessa, Roberto and Guo, Zhen and Ansari, Nirwan},
	journal={IEICE transactions on communications},
	volume={89},
	number={11},
	pages={3120--3123},
	year={2006},
	publisher={The Institute of Electronics, Information and Communication Engineers}
}

@inproceedings{rojas2005combining,
	title={Combining distributed and centralized arbitration schemes for combined input-crosspoint buffered packet switches},
	author={Rojas-Cessa, R and Guo, Zhen and Ansari, N},
	booktitle={Networks, 2005. Jointly held with the 2005 IEEE 7th Malaysia International Conference on Communication., 2005 13th IEEE International Conference on},
	volume={2},
	pages={776--770},
	year={2005},
	organization={IEEE}
}


@inproceedings{rojas2005matching,
	title={Matching schemes with captured-frame eligibility for input-queued packet switches},
	author={Rojas-Cessa, Roberto and Lin, Chuan-bi},
	booktitle={Communications, 2005. ICC 2005. 2005 IEEE International Conference on},
	volume={2},
	pages={972--976},
	year={2005},
	organization={IEEE}
}

@article{gao2013distributed,
	title={Distributed weight matching dispatching scheme in MSM Clos-network packet switches},
	author={Gao, Ya and Qiu, Zhiliang and Zhang, Maosen and Jiang, Yongbo},
	journal={IEEE Communications Letters},
	volume={17},
	number={3},
	pages={580--583},
	year={2013},
	publisher={IEEE}
}

@inproceedings{tian2012sequence,
	title={An in-sequence guaranteed space-memory-memory Clos-network architecture},
	author={Tian, Yupeng and Zhang, Xiaoping and Li, Menghan and Zhang, Haixiang},
	booktitle={ICT Convergence (ICTC), 2012 International Conference on},
	pages={354--359},
	year={2012},
	organization={IEEE}
}

@inproceedings{xia2013practical,
	title={On practical stable packet scheduling for bufferless three-stage Clos-network switches},
	author={Xia, Yu and Chao, H Jonathan},
	booktitle={High Performance Switching and Routing (HPSR), 2013 IEEE 14th International Conference on},
	pages={7--14},
	year={2013},
	organization={IEEE}
}
@inproceedings{kleban2013static,
	title={Static dispatching with internal backpressure scheme for SMM Clos-network switches},
	author={Kleban, Janusz and Suszynska, Urszula},
	booktitle={Computers and Communications (ISCC), 2013 IEEE Symposium on},
	pages={000654--000658},
	year={2013},
	organization={IEEE}
}

@inproceedings{lin2008module,
	title={Module-First Matching Schemes for Scalable Input-Queued Space-Space-Space Clos-Network Packet Switches},
	author={Lin, C-B and Rojas-Cessa, Roberto},
	booktitle={Communications, 2008. ICC'08. IEEE International Conference on},
	pages={5669--5673},
	year={2008},
	organization={IEEE}
}

@inproceedings{hu2011module,
	title={A Module Matched First Dispatching algorithm for MSM Clos-network switches},
	author={Hu, Yanlang and Li, Minqi and Zhou, Quan and Li, Jun and Zhang, Yi and Li, Jingling},
	booktitle={Electronics, Communications and Control (ICECC), 2011 International Conference on},
	pages={4086--4089},
	year={2011},
	organization={IEEE}
}

@inproceedings{xia2012module,
	title={Module-level matching algorithms for MSM Clos-network switches},
	author={Xia, Yu and Chao, H Jonathan},
	booktitle={High Performance Switching and Routing (HPSR), 2012 IEEE 13th International Conference on},
	pages={36--43},
	year={2012},
	organization={IEEE}
}

@inproceedings{chao2012improved,
	title={Improved Static Desynchronization scheme for Clos-network switches},
	author={Chao, Che-Hsi and Hsu, Yarsun},
	booktitle={Computing Technology and Information Management (ICCM), 2012 8th International Conference on},
	volume={2},
	pages={659--664},
	year={2012},
	organization={IEEE}
}

@inproceedings{kleban2007packet,
	title={Packet dispatching algorithms with the static connection patterns scheme for three-stage buffered clos-network switches},
	author={Kleban, Janusz and Santos, Hugo},
	booktitle={Communications, 2007. ICC'07. IEEE International Conference on},
	pages={6319--6324},
	year={2007},
	organization={IEEE}
}

@misc{rojas2015space,
	title={Space-space-memory (SSM) Clos-network packet switch},
	author={Rojas-Cessa, Roberto and Lin, Chuan-Bi and Dong, Ziqian},
	year={2015},
	month=mar # "~31",
	publisher={Google Patents},
	note={US Patent 8,995,456}
}

@inproceedings{liu2015fault,
	title={Fault-tolerant cell dispatching for onboard space-memory-memory Clos-network packet switches},
	author={Liu, Kai and Yan, Jian and Lu, Jianhua},
	booktitle={High Performance Switching and Routing (HPSR), 2015 IEEE 16th International Conference on},
	pages={1--6},
	year={2015},
	organization={IEEE}
}

@article{yu2011out,
	title={Out-of-sequence prevention for multicast input-queuing space-memory-memory clos-network},
	author={Yu, Hao and Ruepp, Sarah and Berger, Michael S},
	journal={IEEE Communications Letters},
	volume={15},
	number={7},
	pages={761--763},
	year={2011},
	publisher={IEEE}
}

@inproceedings{al2008concatenating,
	title={Concatenating Packets in Variable-Length Input-Queued Packet Switches with Cell-Based and Packet-Based Scheduling},
	author={Al-Saber, Nabeel A and Oberoi, Saurabh and Pedasanaganti, Taraka and Rojas-Cessa, Roberto and Ziavras, Sotirios G},
	booktitle={Sarnoff Symposium, 2008 IEEE},
	pages={1--5},
	year={2008},
	organization={IEEE}
}

@unpublished{trident,
	note = "Technical Report TR-NRL-180401: TRIDENT: A load-balancing Clos-network Packet Switch with Queues between Input and Central Stages and In-Order Forwarding \url{http://web.njit.edu/~rojasces/technical-reports/trident171201.pdf}"
}


@inproceedings{pun2002static,
	title={Static round-robin dispatching schemes for Clos-network switches},
	author={Pun, Konghong and Hamdi, Mounir},
	booktitle={High Performance Switching and Routing, 2002. Merging Optical and IP Technologies. Workshop on},
	pages={329--333},
	year={2002},
	organization={IEEE}
}

@inproceedings{jacobson2009networking,
	title={Networking named content},
	author={Jacobson, Van and Smetters, Diana K and Thornton, James D and Plass, Michael F and Briggs, Nicholas H and Braynard, Rebecca L},
	booktitle={Proceedings of the 5th international conference on Emerging networking experiments and technologies},
	pages={1--12},
	year={2009},
	organization={ACM}
}

@inproceedings{pan2017modeling,
	title={Modeling CCN Packet Forwarding Engine},
	author={Pan, Tian and Huang, Tao and Li, Cong},
	booktitle={GLOBECOM 2017-2017 IEEE Global Communications Conference},
	pages={1--6},
	year={2017},
	organization={IEEE}
}

@inproceedings{virgilio2013pit,
	title={PIT overload analysis in content centric networks},
	author={Virgilio, Matteo and Marchetto, Guido and Sisto, Riccardo},
	booktitle={Proceedings of the 3rd ACM SIGCOMM workshop on Information-centric networking},
	pages={67--72},
	year={2013},
	organization={ACM}
}

@inproceedings{jacobson2009voccn,
	title={VoCCN: voice-over content-centric networks},
	author={Jacobson, Van and Smetters, Diana K and Briggs, Nicholas H and Plass, Michael F and Stewart, Paul and Thornton, James D and Braynard, Rebecca L},
	booktitle={Proceedings of the 2009 workshop on Re-architecting the internet},
	pages={1--6},
	year={2009},
	organization={ACM}
}

@inproceedings{wang2009energy,
	title={Energy efficient collision aware multipath routing for wireless sensor networks},
	author={Wang, Zijian and Bulut, Eyuphan and Szymanski, Boleslaw K},
	booktitle={2009 IEEE International Conference on Communications},
	pages={1--5},
	year={2009},
	organization={IEEE}
}

@article{ploumidis2017flow,
	title={Flow allocation for maximum throughput and bounded delay on multiple disjoint paths for random access wireless multihop networks},
	author={Ploumidis, Manolis and Pappas, Nikolaos and Traganitis, Apostolos},
	journal={IEEE Transactions on Vehicular Technology},
	volume={66},
	number={1},
	pages={720--733},
	year={2017},
	publisher={IEEE}
}

@inproceedings{le2011multipath,
	title={Multipath routing design for wireless mesh networks},
	author={Le, Long},
	booktitle={2011 IEEE Global Telecommunications Conference-GLOBECOM 2011},
	pages={1--6},
	year={2011},
	organization={IEEE}
}
